Variable-state Latent Conditional Random Fields for Facial Expression Recognition and Action Unit Detection

Automated recognition of facial expressions of emotions, and detection of facial action units (AUs), from videos depends critically on modeling of their dynamics. These dynamics are characterized by changes in temporal phases (onset-apex-offset) and intensity of emotion expressions and AUs, the appearance of which may vary considerably among target subjects, making the recognition/detection task very challenging. The state-of-the-art Latent Conditional Random Fields (L-CRF) framework allows one to efficiently encode these dynamics through the latent states accounting for the temporal consistency in emotion expression and ordinal relationships between its intensity levels, these latent states are typically assumed to be either unordered (nominal) or fully ordered (ordinal). Yet, such an approach is often too restrictive. For instance, in the case of AU detection, the goal is to discriminate between the segments of an image sequence in which this AU is active or inactive. While the sequence segments containing activation of the target AU may better be described using ordinal latent states, the inactive segments better be described using unordered (nominal) latent states, as no assumption can be made about their underlying structure (since they can contain either neutral faces or activations of non-target AUs). To address this, we propose the variable-state L-CRF (VSL-CRF) model that automatically selects the optimal latent states for the target image sequence. To reduce the model overfitting either the nominal or ordinal latent states, we propose a novel graph-Laplacian regularization of the latent states. Our experiments on three public expression databases show that the proposed model achieves better generalization performance compared to traditional L-CRFs and other related state-of-the-art models.

==> Makefile <==
PROJECT=main

bibtex=bibtex
pdflatex=pdflatex
BIBTEX=$(bibtex) build/main.aux
BUILDTEX=$(pdflatex) \
		 -halt-on-error \
		--output-directory build \
		-aux-directory=build \
		-file-line-error \
		$(PROJECT).tex 


all:
	$(BUILDTEX)
	bibtex build/main.aux
	$(BUILDTEX)
	$(BUILDTEX)

clean:
	rm -rf build/*


==> fig/_graph.tex <==
\begin{figure}[ht]%{{{ FIGURE- GRAPH
    \centering
    \begin{subfigure}[b]{.48\linewidth}
        \resizebox{0.9\textwidth}{!}{%
            \centering
            \tikz{
                \node[obs] (x1) {$\vec{x_1}$}; %
                \node[obs, right=of x1] (x2) {$\vec{x_2}$}; %
                \node[obs, right=of x2] (x3) {$\vec{x_3}$}; %
                \node[obs, right=of x3,xshift=0.7cm] (xt) {$\vec{x_t}$}; %
                \node[latent, above=of x1] (h1) {$\vec{h_1}$}; %
                \node[latent, above=of x2] (h2) {$\vec{h_2}$}; %
                \node[latent, above=of x3] (h3) {$\vec{h_3}$}; %
                \node[latent, above=of xt] (ht) {$\vec{h_t}$}; %
                \node[latent,above=of h3, xshift=0cm] (y) {$y$} ; %
                \edge[-] {x1} {h1} ; %
                \edge[-] {x2} {h2} ; %
                \edge[-] {x3} {h3} ; %
                \edge[-] {xt} {ht} ; %
                \edge[-] {h1} {h2} ; %
                \edge[-] {h2} {h3} ; %
                \edge[-,dashed] {h3} {ht} ; %
                \edge[-] {h1} {y} ; %
                \edge[-] {h2} {y} ; %
                \edge[-] {h3} {y} ; %
                \edge[-] {ht} {y} ; %
            }
        }
        \caption{H-CRF\cite{hcrf06}/H-CORF\cite{hcorf}}
        \label{fig:H-CRF}
    \end{subfigure}%
    \begin{subfigure}[b]{.48\linewidth}
        \resizebox{0.9\textwidth}{!}{%
            \centering
            \tikz{
                \node[obs] (x1) {$\vec{x_1}$}; %
                \node[obs, right=of x1] (x2) {$\vec{x_2}$}; %
                \node[obs, right=of x2] (x3) {$\vec{x_3}$}; %
                \node[obs, right=of x3,xshift=0.7cm] (xt) {$\vec{x_t}$}; %
                \node[latent, above=of x1] (h1) {$\vec{h_1}$}; %
                \node[latent, above=of x2] (h2) {$\vec{h_2}$}; %
                \node[latent, above=of x3] (h3) {$\vec{h_3}$}; %
                \node[latent, above=of xt] (ht) {$\vec{h_t}$}; %
                \node[latent,above=of h3, xshift=0cm] (nu) {$\nu$} ; %
                \node[latent,above=of nu, xshift=0cm] (y) {$y$} ; %
                \edge[-] {x1} {h1} ; %
                \edge[-] {x2} {h2} ; %
                \edge[-] {x3} {h3} ; %
                \edge[-] {xt} {ht} ; %
                \edge[-] {h1} {h2} ; %
                \edge[-] {h2} {h3} ; %
                \edge[-,dashed] {h3} {ht} ; %
                \edge[-] {h1} {nu} ; %
                \edge[-] {h2} {nu} ; %
                \edge[-] {h3} {nu} ; %
                \edge[-] {ht} {nu} ; %
                \edge[-] {nu} {y} ; %
            }
        }
        \caption{VSL-CORF\cite{hcorf}}
        \label{fig:H-CRF}
    \end{subfigure}
    \caption{The graphical model of the (a) traditional Latent CRF models (e.g., H-CRF\cite{}/H-CORF\cite{}), and (b) proposed VSL-CRF model. In H-CRF/H-CORF, the latent states $h$, relating the observation sequence ${\bf x}=\{x_1,\dots,x_T\}$ of the input image features (e.g., the locations of fiducial facial points or apperance-based descriptors extracted from each frame in an image sequence) to the target label $y$ (e.g., the emotion-specific label, or the AU activation 0/1), are allowed to be either nominal or ordinal for all image sequences in the training dataset. By contrast, in the VSL-CRF, the latent variable $\nu$ is introduced, which allows the model to  perform automatic selection of the optimal latent states for each sequence (nominal or ordinal), resulting in a more flexible model for the target task.}
    \label{fig:graph}
\end{figure}%}}}


==> fig/fb_au_activity.tex <==
\begin{figure*}[ht]%{{{ FIGURE- GRAPH
    \centering
  \includegraphics[width=1\linewidth]{./fig/AU_Chart.png}
  \caption{
      Frame-based predictions of AU1 (Inner Brow Raiser) and AU6 (Cheek Raiser) from the DISFA database. 
      Sliding windows with the optimal window size around each target frame were used in order obtain the per-frame predictions (red dashed line).
      \label{fig:au_chart}
  }
\end{figure*}%}}}


==> tab/SB_FERA_EMO.tex <==
\begin{table}[t]%{{{
\footnotesize
\rowcolors{2}{white}{tablegray}
\begin{tabularx}{\linewidth}{l|XXXXXX}
\rowcolor{tablegray}
\toprule
Emotion  & SVM  & HCRF & HCORF & VSLm & VSLd    & VSLem      \\
\midrule 
Anger    & 64.5 & 54.8 & 61.2  & 71.1   & 71.0      & \bf{74.4}  \\
Fear     & 46.7 & 50.0 & 50.1  & 60.1   & 66.7      & \bf{69.8}  \\
Joy      & 74.1 & 74.1 & 63.0  & 70.3   & \bf{81.5} & 77.8       \\
Relief   & 53.3 & 63.3 & 63.1  & 63.2   & 53.3      & 50.2       \\
Sadness  & 40.0 & 70.0 & 53.5  & 56.7   & 70.0      & 69.8       \\
\midrule 
Avg      & 55.7 & 62.4 & 58.2  & 64.3   & \bf{68.5} & 68.4       \\
\bottomrule
\end{tabularx}
\label{tab:fera_emo}
\caption{Per-sequence classification rate on the \textbf{GEMEP-FERA} emotion database}
\end{table}%}}}

%\begin{table}[t]%{{{
%\footnotesize
%\rowcolors{4}{white}{tablegray}
%\begin{tabularx}{\linewidth}{l|XXXXXX|X}
%\toprule
%Emotion  & SVM  & HCRF & HCORF & VSLmax & VSLdir    & VSLem     & CLM                   \\
         %&      &      &       &        &           &           & \cite{chew2011person} \\
%\midrule 
%Anger    & 64.5 & 54.8 & 61.2  & 71.1   & 71.0      & \bf{74.4} & 43.0                  \\
%Fear     & 46.7 & 50.0 & 50.1  & 60.1   & 66.7      & \bf{69.8} & 20.0                  \\
%Joy      & 74.1 & 74.1 & 63.0  & 70.3   & \bf{81.5} & 77.8      & 75.0                  \\
%Relief   & 53.3 & 63.3 & 63.1  & 63.2   & 53.3      & 50.2      & \bf{88.0}             \\
%Sadness  & 40.0 & 70.0 & 53.5  & 56.7   & 70.0      & 69.8      & \bf{87.0}             \\
%\midrule 
%Avg      & 55.7 & 62.4 & 58.2  & 64.3   & \bf{68.5} & 68.4      & 62.6                  \\
%\bottomrule
%\end{tabularx}
%\caption{Experimental resutls on the GEMEP-FERA database. The table shows the classification rate for emotion detection.}
%\end{table}%}}}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


